U-RED: Unsupervised 3D Shape Retrieval and Deformation for Partial Point Clouds

In this paper, we propose U-RED, an Unsupervised shape REtrieval and Deformation pipeline that takes an arbitrary object observation as input, typically captured by RGB images or scans, and jointly retrieves and deforms the geometrically similar CAD models from a pre-established database to tightly match the target. Considering existing methods typically fail to handle noisy partial observations, U-RED is designed to address this issue from two aspects. First, since one partial shape may correspond to multiple potential full shapes, the retrieval method must allow such an ambiguous one-to-many relationship. Thereby U-RED learns to project all possible full shapes of a partial target onto the surface of a unit sphere. Then during inference, each sampling on the sphere will yield a feasible retrieval. Second, since real-world partial observations usually contain noticeable noise, a reliable learned metric that measures the similarity between shapes is necessary for stable retrieval. In U-RED, we design a novel point-wise residual-guided metric that allows noise-robust comparison. Extensive experiments on the synthetic datasets PartNet, ComplementMe and the real-world dataset Scan2CAD demonstrate that U-RED surpasses existing state-of-the-art approaches by 47.3%, 16.7% and 31.6% respectively under Chamfer Distance.

==> Sections/1intro.tex <==
\section{Introduction}
Semantic scene perception~\cite{nie2020total3dunderstanding, zhang2021holistic} involves the decomposition of the scene into its constituent objects, understanding and reconstructing all the detected objects, and putting them into place to formulate a holistic scene representation.

To obtain a high-quality corresponding 3D model matching a given noisy and partially-observed target object scan from the real world is a laborious but meaningful task. 
This enables 3D perception of a scanned scene characterized as a compact and clean CAD representation \cite{gumeli2022roca}. 
However, existing neural-network-based generative methods lack the capability to guarantee the fidelity, rich details, and overall quality of created 3D models \cite{tatarchenko2019single}. 
Moreover, real-world scanning data often meets incomplete areas, occluded parts, and noisy points. 
These complicated scenarios further raise the difficulty level of this task.

Many prior approaches follow a pipeline that first retrieves a stored CAD model from a database and then deforms it to match the target object scanning. 
However, most of them focus on only one sub-problem of the pipeline, retrieving an proper mesh from a database \cite{dahnert2019joint}\cite{nan2012search}\cite{uy2020deformation} or deforming a appointed source model to fit the target \cite{yifan2020neural}\cite{wang20193dn}\cite{jiang2020shapeflow}, and they finally combine the two stages to create a  3D model. 
The separated and static approaches need to face the problem of accumulated error of two cascaded stages, and ignore the possibility that a database shape could produce the best match after proper deformation, which significantly reduce their generalization ability. 
Thus, these methods may yield decent performance on selected synthetic datasets, but often fail to deal with noisy and even partial scanning, which is the frequent circumstance in the real world.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figs/Pipeline.pdf}
    \caption{}
    \label{fig:teaser}
\end{figure}



To address the problem, there are some emerged methods aiming at joint optimizing the retrieval and the deformation step. \cite{schulz2017retrieval} and \cite{uy2020deformation} propose to explicitly consider deformation-aware retrieval.
However, their deformation modules are fixed and necessitate time-consuming and manually-specified optimization. 
\cite{uy2021joint} presents a joint training strategy with a combined loss to make the network aware both retrieval and deformation simultaneously.
Since strong supervised by the ground truth target 3D model and necessitating input with full scanned point clouds, \cite{uy2021joint} performs decently in the synthetic dataset. 
Nevertheless, when migrating to noisy, partially-observed and sometimes unseen objects in real-world scanning, this supervised method often fails. 
Moreover, the joint learning technique they propose is only to add an explicit probabilistic retrieval weight for final deformation loss, which seems to be naive to construct effective connection between retrieval and deformation result.

In this paper, we propose Un-3RD, an \textbf{Un}supervised joint \textbf{3}D shape \textbf{R}etrieval and \textbf{D}eformation to effectivelly handle with noisy, partially-observed and unseen objects in real-world scanning. 
Our unsupervised geometry-guided joint training pipeline empowers the proposed network much stronger generalization ability for noisy and unseen adaptation, since it does not enforces the network to remember all target shapes but enlightens it to attend to geometric consistency between partial and full objects. 
Meanwhile, Un-3RD does not demand numerous ground truth target CAD models inaccessible under many circumstances, while only use economically obtained synthetic full point clouds to guide the optimization by a proposed complementary geometry-guided training technique. 
The gained strong generalization capability by this unsupervised geometry-guided training strategy makes Un-3RD easy to directly handle the complicated real-world scanning, yielding impressive quantitative and qualitative effects with only zero-shot transferring.

Noticing drawbacks of \cite{uy2021joint} of over-simplified joint network designing and complicated alternative training tricks, Un-3RD adopts a novel integrated latent-embedding deformation-aware retrieval technique and a graph attention based point matching and deformation architecture. 
To optimize our joint pipeline efficiently, we design several tightly-coupled losses to exploit implicit connection between shape retrieval and deformation process. Our proposed retrieval technique abandons the explicit classification probability adopted by \cite{uy2021joint}\cite{nan2012search}. On the contrary, we use a retrieval-sensitive deformation residual loss to evaluate our retrieval architecture, which leads the retrieval model pay more attention to final target deformation result rather than only produce a classification score. The graph attention based point matching and deformation architecture is empowered to exploit geometric connection between different segmented part of the scanned source objects. Meanwhile, it extracts aggregated local structure feature of both target and source point clouds for more precise points matching and deformation, rather than merely consider reconstruction latent codes as previous methods.

Our main contribution are summerized as follows:
\begin{itemize}
\item 
We propose a novel unsupervised approach Un-3RD, capable of conducting precise joint 3D shape retrieval and deformation when facing noisy, partially-observed and unseen scanning in real world, yielding state-of-the-art performance in both synthetic ShapeNet \cite{chang2015shapenet} and real Scan2CAD \cite{avetisyan2019scan2cad}.
\item
We design an effective unsupervised complementary geometric-
guided training pipeline, enabling only using synthetic full point clouds and their generated parts to train the network aware of geometry consistency between full and partial scanning, and gaining impressive effects when zero-shot adapted to real noisy scanning.
\item
We present an integrated latent-embedding deformation-aware retrieval technique and a graph attention based point matching and deformation architecture for exploitation to deeper implicit connection of shape retrieval and deformation.
\end{itemize}


==> Sections/3method.tex <==
\section{Method}
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{Figs/Pipelinev2.pdf}
    \caption{}
    \label{fig:pipeline}
\end{figure*}

\subsection{Overview}
Un-3DR provides an efficient pipeline to conduct joint shape retrieval and deformation, processing noisy scene point clouds from scanning or depth estimation via RGB input to handle with 3D scene understanding task by generating a clean and compact deformed CAD representation, as \ref{fig:pipeline} shows. It follows an unsupervised pipeline to gain maximized generalization ability when facing noisy, heavily-occluded, partially-observed and sometimes unseen object scanning. 

For a color image from a real-world scene, we adopt a MaskRCNN \cite{he2017mask} to segment the object region of interest, and then use the mask for depth scanning or estimation to generate target partially-observed point clouds $T_p$.
$T_p$ is uniformly sampled to 1024 points for convenience of process. 
$T_p$ and corresponding source shapes $\{S\}$ in database are first fed to partial encoder and source encoder for latent embeddings extraction. 
The latent target embeddings $F_{tp}$ and source embeddings $\{F_s\}$ are shared by the reconstruction head, retrieval residual head and deformation head, ensuring the consistency of outputs of different heads via well-designed losses during training stage. 
Un-3DR presents an unsupervised consistent geometric-guided training technique with not only mutual geometric supervision by exploiting constraints among different heads, but also a complementary branch with full point clouds input, making partial inference branch aware of the whole shape of the target instance. 
This technique enhances the geometric representation ability considering both retrieval and deformation tasks.

During inference stage, only the retrieval residual head and deformation head are used for tightly-coupled joint shape retrieval and deformation. 
We design a deformation-aware residual-guided retrieval technique. 
The residual field estimated by the retrieval residual head describes the discrepancy between deformed source shapes and the input target, and executes soft retrieval by measuring the residuals. 
For deformation head, we presents a graph attention based deformation architecture to sufficiently exploit the relationship between source parts in the database and the target shape using the graph attention mechanism. 
Via joint shape retrieval and deformation, a clean high-quality CAD model  matching the input point clouds is generated. 
This deformed model is aligned to scene coordinate to generate the final compact scene representation. 

\subsection{Deformation-aware Residual-guided Retrieval}\label{DRR}
To solve the problem of two separated stages for shape retrieval and deformation, we design a tightly-coupled deformation-aware residual-guided retrieval technique to enable joint retrieval and deformation inference. 

We introduce a retrieval residual network to generate deformation-aware retrieval residual field, describing the discrepancy between deformed source shapes and the input point clouds. 
The retrieval residual network $D_{res}$ is a 5-layer MLP with BN layers, with input of concatenation of $F_{tp} \in \mathbb{R}^{512}$ and $F_s \in \mathbb{R}^{512}$. 
It generates the residual direction field $d \in \mathbb{R}^{1024 \times 3}$ for all 1024 points of deformed source shapes $DS$ by the graph attention based deformation module introduced in \ref{GABD}. 
\begin{equation}
d = D_{res}(F_{tp}, F_s)
\end{equation}
The residual direction $d^i \in \mathbb{R}^3$ for $i$-th point needs to satisfy $T_p^i = DS^i \oplus d^i$ as much as possible, since it measures geometric likelihood or discrepancy between the deformed source shapes and the input point clouds. 
Here, $\oplus$ indicates pointwise addition for $i$-th K-nearest neighbors matching. To effectively constrain $d$, we propose a retrieval residual loss
\begin{equation}
L_{re-residual} = \frac{1}{N} \sum_{i=1}^{N} |DS^i + d^i - KNN_i(T_p)|
\end{equation}
where $KNN_i$ indicates the $i$-th K-nearest neighbors matching for $DS^i$ and $T_p$, $N$ is the total number of input and output point clouds. 

During inference, we harness the residual direction field $d$ to score every source shape and get top-k soft retrievals as the final results. 
This procedure can be expressed as
\begin{equation}
\{S_{re}\} = \{S_k | k \in argminK(\sum_{i=1}^{N}||d^i_k||_2)\} 
\end{equation}
where $\{S_{re}\}$ means final set of retrieved source shapes with the capacity of $K$, $d^i_k$ indicates the residual vector for $i$-th point of $k$-th input source. The retrieval score is the sum of Euclidean norm for $d^i_k$, which means we need to find the top suitable source shapes possessing the least discrepancy between their deformed shapes and the target input. As \cite{uy2021joint}, after yielding softly retrieved $\{S_{re}\}$, we feed their corresponding latent embeddings to deformation head to gain the final deformed shape.  

This deformation-aware learning procedure enforces the retrieval residual head significantly considers the deformation results when predicting corresponding residual field and then scoring every source to make retrieval decision. 
This design is more tightly-coupled compared to previous joint retrieval and deformation methods since 1. the latent embeddings $D_{res}$ uses are integrally supervised by multi-tasks including both deformation and retrieval; 2. the residual field used for retrieval task is constrained by $L_{re-residual}$ considering deformed source shapes as supervision.

\subsection{Graph Attention Based Deformation}\label{GABD}
We present a graph attention based architecture inspired by \cite{thekumparampil2018attention} for deformation task to exploit geometric and structural relationships among different parts of input point clouds. This module predicts deformation parameters consisting of translation and axis-aligned scaling for each part in a source model, respecting the part-to-part connectivity of the source shape defined in the database. 

The latent embeddings $F_{tp}$ and $F_s$ are fed to a 3-layers MLP to generate global node coding $N_{g}$ for the graph network. Simultaneously, pointwise $F_s$ is divided by part masks provided by source database, and then fed to another 3-layers MLP to generate part node coding $N_{p}$. In the graph attention network, messages of $N_{g}$ and $N_{p}$ are mutually passed through self-attention and cross-attention mechanisms as adopted in \cite{guo2021pct}. Concretely, the node message passing process is illustrated as 
\begin{equation}
N'_i = N_i + MLP(MHA(Q, K, V))
\end{equation}
where $i = g, p$, $MHA$ refers to multi-head attention mechanism. For self-attention mechanism, $Q, K, V = N_i$, while for cross-attention mechanism, $Q = N_i$ but $K, V = N_p, i = g; K, V = N_g, i = p$. Such self-attention and cross-attention message passing are conducted alternatively for both $N_{g}$ and $N_{p}$, and are repeated by two times during implementation. The message passing procedure between part and global nodes significantly helps the network exploit relationships between different geometric parts of source and target shapes, and exchange information between structural parts and the corresponding full shape, leading a superior geometry-aware and part-aware deformation.

The deformation module is guided by chamfer loss $L_{chamfer}$, between output deformed point clouds and input target point clouds. Further, we also utilize a symmetry loss $L_{symmetry}$ as adopted in \cite{uy2021joint} to enforce bilateral symmetry of the output deformed shapes as regularization.


\subsection{Unsupervised Consistent Geometry-guided Training}\label{UCGT}
Our unsupervised geometry-guided training technique aims at getting rid of limitation of access to clean ground truth target models, and gaining strong generalization ability by enforcing networks to learn geometry features and relationships between paritial and full structures rather than simply to remember all possible target shapes. Thus, we design multiple heads to generate geometry-aware latent embeddings for target and source shapes, ensuring the consistency between outputs of different heads and providing mutual geometric supervision via well-designed losses. Moreover, we introduce a complementary branch with full point clouds input, making partial inference branch aware of the whole shape of the target instance.

\textbf{Latent Embeddings with Multi-tasks Consistency.}
Without ground truth target supervision, Un-RED needs to construct effective self-supervision exploiting geometric relationships among partial target input, full target input, self-reconstructed target shape and final deformed shape. 
Mutual geometric supervision via well-designed losses is used to guide target embeddings $F_{tp} \in \mathbb{R}^{512}$  extracted by a VN-PointNet \cite{deng2021vector} partial encoder, as well as sources embeddings $F_s \in \mathbb{R}^{512}$ extracted by a VN-PointNet \cite{deng2021vector} source encoder.
As introduced in \ref{DRR}, $L_{re-residual}$ makes aware of the latent embeddings $F_{tp}$ and $\{F_s\}$ to exploit connection of deformation and retrieval tasks. \ref{GABD} presents $L_{chamfer}$ and $L_{symmetry}$ to directly pass geometric information of deformation to the latent embeddings. Besides retrieval residual head and deformation head used during inference, we also design several supplementary modules to provided enough geometric constraints during training stage, including partial reconstruction head, source reconstruction head and a dual branch with full point clouds input. Partial reconstruction head $D_{PRecon}$ and source reconstruction head $D_{SRecon}$ benefits $F_{tp}$ and $\{F_s\}$ respectively from enabling it with strong geometric representation capability to recover input target partial shape and source shapes as much as possible. $D_{PRecon}$ and $D_{SRecon}$ possess the same architecture of 5-layer MLP with BN layers. The reconstruction loss for both heads shares the same format:
\begin{equation}
L_{recon} = ||\hat{P_{tp/s}} - P_{tp/s}||_2^2
\end{equation}
where $\hat{P_{tp/s}}$ means the reconstructed point clouds for $T_p$ or ${S}$, $P_{tp/s}$ means the input point clouds for $T_p$ or ${S}$.

\textbf{Learning Awareness of Full Shape.}
Clean deformed target shapes are hard to get for training, which is solved by introducing a dual branch with full target point clouds input in Un-RED, teaching the unsupervised model aware of full input shape to make more precise deformation predictions. Note that the full target point clouds of synthetic datasets we use are merely the network input of previous method \cite{uy2021joint}, basically different from their necessity to clean deformed model parameters for target objects during training. The dual branch with full target point clouds input possesses the same architecture and losses with partial pipeline introduced above, with outputs including full reconstruction, retrieval residual field and deformed shape. The additional supervision provided by the full branch mainly lies on the deformed shape with full input, by the loss
\begin{equation}
L_{consistency} = ||P_{deformedF} - P_{deformedP}||_2^2
\end{equation}
where $P_{deformedF}$ is deformation point clouds generated by the full branch and $P_{deformedP}$ is the inference output deformation result with only partially-observed target point clouds.

Aggregating all losses for joint retrieval and deformation introduced above, the final loss for our unsupervised training could be written by
\begin{equation}
\begin{aligned}
L = \lambda_{chamfer}L_{chamfer} + \lambda_{symmetry}L_{symmetry} + \\ \lambda_{re-residual}L_{re-residual} + \lambda_{recon}L_{recon} + \\ \lambda_{consistency}L_{consistency}
\end{aligned}
\end{equation}

\textbf{Synthetic Occlusion Simulation and Partial Scanning Generation.}
Since Un-RED is trained on synthetic dataset and makes inference directly on real-world dataset with zero-shot adaptation, simulating reasonable occlusion to generate real enough partial scanning is significant during the training stage. The partial point clouds input of the network during training are generated through the combination of three simulation techniques, including ball occlusion, plane occlusion and random mask occlusion. Such combination of the three occlusion simulations could present much of the circumstances in real world. For specific implementation details, please refer to our supplementary material.


==> Sections/4exp.tex <==
\section{Results}
\subsection{Experimental Setup}
\textbf{Datasets.}
We train Un-RED on three furniture categories of the synthetic ShapeNet \cite{chang2015shapenet} dataset chairs, tables and cabinets. For our database of source models, we respectively adopt manually and automatically-segmented shapes from two different datasets. Manually-segmented shapes come from the finest level of PartNet hierarchy \cite{mo2019partnet}, selecting $10\%$ data as our sources (500 chairs, 793 tables and 127 cabinets). Automatically-segmented shapes come from two classes in ComplementMe \cite{sung2017complementme} (chairs and tables), and we pick 200 random models for each. We remove the selected sources and using remaining as training ($80\%$) and testing targets ($20\%$) for synthetic scenario. Note that we only use targets point clouds rather than specific parametric ground truth deformed target shapes since our unsupervised setting. The partial target point clouds for training and testing are generated by our synthetic occlusion simulation technique introduced in \ref{UCGT}. After trained by synthetic datasets, Un-RED can directly generalize to real-world scenario. We use segmented scene scanning of chairs, tables and cabinets in Scan2CAD \cite{avetisyan2019scan2cad} dataset to test the performance when facing real-world noisy and partially-observed point clouds. All sources and targets are represented as 1024 points after uniform sampling. During training, we randomly choose several source shapes from the database for one batch. Training is end-to-end rather than follows an alternative manner as \cite{uy2021joint}. During testing, our graph attention based deformation module only process the top 10 retrieved sources by the deformation-aware residual-guided retrieval module. The average chamfer distance between the deformed sources and the ground truth targets are reported as evaluation metrics. Some network architecture details and training settings are shown in our supplementary material.


\subsection{Real-world Scenario}
\begin{table}[]
\setlength\tabcolsep{1pt}
\begin{center}
\begin{tabular}{cccc}
\hline
Method            & Chair(3544)          & Table(2079)           & Cabinet(781)\\
\hline
Uy et al. \cite{uy2021joint} & 3.36 & 6.65 & 7.26
 \\
ROCA* \cite{gumeli2022roca} &4.24  &14.97  & 15.92
 \\
ROCA* \cite{gumeli2022roca} + De &6.99  &8.10  & 13.08
 \\
Ours        & \textbf{2.89} & \textbf{3.16} & \textbf{5.95} \\
\hline
\end{tabular}
\end{center}
\caption{Joint retrieval and deformation results on real Scan2CAD \cite{avetisyan2019scan2cad} dataset (chamfer distances, $\times10^{-2}$). The number refers to the total instance number of the category.}
\label{tab:roca_result}
\end{table}

We directly test Un-RED trained on synthetic ShapeNet \cite{chang2015shapenet} dataset with PartNet \cite{mo2019partnet} segmentation on real-world Scan2CAD \cite{avetisyan2019scan2cad} dataset. Results shown in Tab. \ref{tab:roca_result} demonstrate that Un-RED yields the most precise deformed CAD model to represent the real world scene, due to its best generalization ability enabled by appropriate module design and effective unsupervised consistent geometry-guided learning.

Concretely, compared with \cite{uy2021joint} which gains decent results on synthetic scenario, the average chamfer distances of the deformed models by Un-RED decrease by 14.0\%, 52.5\% and 18.0\% for three categories respectively. -------------------------Visualization---------------------- Note that for fair comparison, we train \cite{uy2021joint} by our partial synthetic objects consistent with those fed to Un-RED training procedure to try to teach it get accustomed to partially observed point clouds. Still, it gains inferior performance due to lack of generalization by its supervised manner which only teach it to remember all shapes in training dataset.

Further, we re-implement ROCA \cite{gumeli2022roca}, training it on the same synthetic ShapeNet dataset with PartNet segmentation and testing it on Scan2CAD. The result of the reproduced ROCA with only retrieval head is exhibited as ROCA* in Tab. \ref{tab:roca_result}. We further add a deformation head with the same architecture as we adopt in Sec. \ref{GABD} for fair comparison, as is shown by ROCA* + De in Tab. \ref{tab:roca_result}. The chamfer distances yielded by Un-RED decrease by 31.8\%, 78.9\% and 62.2\% respectively compared with ROCA*, and 58.7\%, 61.0\% and 54.5\% compared with ROCA* + De. Actually, ROCA seems to be failed to conduct such a domain adaptation and performs poor generalization capability, although it performs decently when tested on synthetic dataset as Tab. \ref{tab:shapenet_result} shows. We check it carefully during experiments and find that the reason comes from its improper retrieval process by comparing the Euclidean distance of target and source CADs in feature space directly. When directly tested under similar circumstance as training dataset, the feature extracted by encoders can approximately measure the similarity of target and source objects. However, when tested on unseen real-world dataset, encoders of ROCA struggle to produce meaningful embeddings since they have never seen such shapes before, leading huge gaps of the Euclidean distance of target and source CADs and making wrong retrieval decisions. Although adding a deformation head to ROCA, the performance of ROCA* + De still far from satisfactory because ineffective retrieval results significantly increase the difficulty of deformation module. On the contrast, our deformation-aware residual-guided retrieval technique explicitly considers retrieval operation on deformed results end with the help of the residual prediction head. Thus, it can release the negative effects of noisy embeddings and perform robustly for real-world scanning. 

\subsection{Synthetic Scenario}
\begin{table}[]
\setlength\tabcolsep{2pt}
\begin{center}
\begin{tabular}{cccc}
\hline
Method            & Chair(1207)          & Table(1430)         & Cabinet(231)\\
\hline
Uy et al. \cite{uy2021joint} & 2.02 & 2.32 & 2.63
 \\
ROCA* \cite{gumeli2022roca} &2.50  &2.72  & 3.86
\\
ROCA* \cite{gumeli2022roca} + De &3.80  &3.87  &2.82 
 \\
Ours        & \textbf{0.95} & \textbf{1.33} & \textbf{1.30}\\
\hline
Uy et al. \cite{uy2021joint} & 2.08 & 2.66 & -
\\
Ours        & \textbf{1.68} & \textbf{2.26} & -\\
\hline
\end{tabular}
\end{center}
\caption{Joint retrieval and deformation results on synthetic ShapeNet \cite{chang2015shapenet} dataset, top block is with manually-segmented PartNet \cite{mo2019partnet} and bottom block is with automatically-segmented ComplementMe \cite{sung2017complementme} (chamfer distances, $\times10^{-2}$).}
\label{tab:shapenet_result}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{Figs/Exp_shape_final.pdf}
    \caption{Visualization effects on ShapeNet \cite{chang2015shapenet} dataset with PartNet \cite{mo2019partnet} segmentation. Qualitative comparison with \cite{uy2021joint} demonstrates that our Un-RED performs more robustly, gains more accurate retrieval and more precise deformation when facing with partially observed point clouds.}
    \label{fig:exp_shape}
\end{figure}

The objective of Un-RED is using proper unsupervised training procedure to enhance the generalization ability to handle with noisy and partial input in real-world scenario, still, for fair comparison with existing methods \cite{uy2021joint, gumeli2022roca}, we conduct several experiments on synthetic datasets. The relative results show that our Un-RED also gains superior performance at a large margin when facing occlusion and partially-observed point clouds in synthetic scenario.

In ShapeNet with PartNet segmentation, Un-RED surpasses \cite{uy2021joint} by 53.0\%, 42.7\% and 50.6\% on chair, table and cabinet categories respectively, exceeds ROCA* by 62\%, 51.1\% and 66.3\% and ROCA* + De by 75.0\%, 65.6\% and 53.9\% respectively.  In ShapeNet with ComplementMe segmentation, Un-RED still surpasses \cite{uy2021joint} by 19.2\% and 15.0\% for chair and table categories respectively. Fig. \ref{fig:exp_shape} exhibits the qualitative visualization comparison between our Un-RED and \cite{uy2021joint}. Our Un-RED possesses more accurate retrieval results (the chair in the $1^{st}$ row) and stronger deformation capability (the table in the $5^{th}$ row). Due to our geometry consistent learning, effective module design and tightly-coupled joint retrieval and deformation technique, Un-RED yields the best quantitative metrics and visual effects.

\subsection{Ablation Studies}

\begin{table}[]
\setlength\tabcolsep{8pt}
\begin{center}
\begin{tabular}{cccc}
\hline
Method            & Chair          & Table           & Cabinet\\
\hline
Uy et al. \cite{uy2021joint} & 2.83 & 2.47 & \textbf{4.56}
 \\
Ours        & \textbf{2.05} & \textbf{1.43} & 5.27\\
\hline
Uy et al. \cite{uy2021joint} & 1.43 & 1.48 & 1.79
 \\
Ours        & \textbf{0.70} & \textbf{0.69} & \textbf{0.74}\\
\hline
\end{tabular}
\end{center}
\caption{Deformation results with oracle retrieval on real Scan2CAD \cite{avetisyan2019scan2cad} dataset (top block) and synthetic ShapeNet \cite{chang2015shapenet} dataset with manually-segmented PartNet \cite{mo2019partnet} (bottom block) (chamfer distances, $\times10^{-2}$).}
\label{tab:deform_result}
\end{table}

\begin{table}[]
\setlength\tabcolsep{6pt}
\begin{center}
\begin{tabular}{cccc}
\hline
Method            & Chair          & Table           & Cabinet\\
\hline
Uy et al.* \cite{uy2021joint}  &7.39  &6.00  &15.24  \\
Ours        &\textbf{2.89} & \textbf{3.16} & \textbf{5.95}\\
\hline
Uy et al.* \cite{uy2021joint}  &2.84  &5.17  & 4.66
 \\
Ours        &\textbf{0.95}&  \textbf{1.33}& \textbf{1.30} \\
\hline
\end{tabular}
\end{center}
\caption{Retrieval ablations on real Scan2CAD \cite{avetisyan2019scan2cad} dataset (top block) and synthetic ShapeNet \cite{chang2015shapenet} dataset with manually-segmented PartNet \cite{mo2019partnet} (bottom block) (chamfer distances, $\times10^{-2}$).}
\label{tab:retrieval_ablation_result}
\end{table}

\begin{table}[]
\setlength\tabcolsep{6pt}
\begin{center}
\begin{tabular}{cccc}
\hline
Method            & Chair          & Table           & Cabinet\\
\hline
w/o $L_{consistency}$  &3.57  &5.56  & 6.54
 \\
w/o $L_{recon}$  &4.47  &5.03  &9.11 \\
w/o $L_{re-residual}$  &2.95  &5.32  &19.6 \\
Ours        &\textbf{2.89} & \textbf{3.16} & \textbf{5.95} \\
\hline
w/o $L_{consistency}$  &1.01&  1.41&  2.25
 \\
w/o $L_{recon}$  &1.37&  1.63&  1.51 \\
w/o $L_{re-residual}$  &2.02&  1.77&  1.54 \\
Ours        &\textbf{0.95}&  \textbf{1.33}& \textbf{1.30} \\
\hline
\end{tabular}
\end{center}
\caption{Unsupervised training ablations on real Scan2CAD \cite{avetisyan2019scan2cad} dataset (top block) and synthetic ShapeNet \cite{chang2015shapenet} dataset with manually-segmented PartNet \cite{mo2019partnet} (bottom block) (chamfer distances, $\times10^{-2}$).}
\label{tab:training_ablation_result}
\end{table}

\begin{table}[]
\setlength\tabcolsep{6pt}
\begin{center}
\begin{tabular}{cccc}
\hline
Occlusion Proportion           & Chair          & Table           & Cabinet\\
\hline
0\%  &0.77  &1.34  &1.18  \\
25\%  &0.86  &1.33  &1.23  \\
50\%  &0.95  &1.33 &1.30 \\
75\%  &1.09  &2.21 &1.65 \\
\hline
\end{tabular}
\end{center}
\caption{Occlusion proportion ablations on synthetic ShapeNet \cite{chang2015shapenet} dataset with manually-segmented PartNet \cite{mo2019partnet} (bottom block) (chamfer distances, $\times10^{-2}$).}
\label{tab:partial_ablation_result}
\end{table}

We conduct several ablation studies for deformation ability (Tab. \ref{tab:deform_result}), retrieval ability (Tab. \ref{tab:retrieval_ablation_result}), effectiveness of unsupervised training techniques (Tab. \ref{tab:training_ablation_result}) and robustness to input occlusion proportion (Tab. \ref{tab:partial_ablation_result}). These ablation studies further demonstrate the effectiveness of Un-RED to handle with partial points in both real-world and synthetic scenario.

Tab. \ref{tab:deform_result} exhibits the chamfer distance metrics of Un-RED and \cite{uy2021joint} with oracle retrievals, which means to retrieval every source shape in the database and record the minimum chamfer distances after deformation. This ablation mainly demonstrates the absolute deformation ability of our graph attention based deformation module. Relative results show that when only considering deformation ability, the Un-RED surpasses \cite{uy2021joint} by 42.1\% at maximum (table) in real-world Scan2CAD and 53.4\% at maximum (table) in synthetic PartNet.

Tab. \ref{tab:retrieval_ablation_result} shows the chamfer distance metrics of Un-RED with different retrieval techniques. Uy et al.* means to use their probabilistic soft retrieval strategy \cite{uy2021joint} and keep other modules of Un-RED remained. This ablation verifies the effectiveness of the proposed deformation-aware residual-guided retrieval module. Since it enforces the
retrieval residual head significantly considering the deformation results during training stage, our proposed technique performs more tightly-coupled joint retrieval and deformation results and exceeds Uy et al.* by 61.0\% (cabinet) at maximum in Scan2CAD and 74.3 (table) at maximum in PartNet.

Tab. \ref{tab:training_ablation_result} illustrates the effectiveness of our proposed losses for unsupervised training stage.

Tab. \ref{tab:partial_ablation_result} measures the robustness of our method when facing with different occlusion proportion of input partially-observed point clouds.


